Saving Tokens in Rollout Control with Token Bucket Specification

We consider a communication network over which transmissions must fulfill the so-called token bucket traffic specification, with a rollout (i.e., predictive) controller that both schedules transmissions and computes the corresponding control values. In the token bucket specification, a transmission is allowed if the current level of tokens is above a certain threshold. Recently, it has been shown that having a full bucket at the time of a set point change significantly improves the control performance as compared to when the bucket level is low. In this work, we develop mechanisms that guarantee that the bucket fills up after the controlled plant has converged to a set point. To do this, we consider two different setups. First, we consider that all transmissions over the network must fulfill the token bucket specification and show convergence to the upper sector of the bucket by adding a slight terminal cost on the bucket level. Afterwards, we consider a modified network which additionally features a direct link over which transmissions need not fulfill the token bucket specification. In this setup, we prove convergence of the bucket level exactly to the upper rim. These mechanisms enable a similar level of flexibility as event-triggered control: In converged state, little communication is used while in precarious operating conditions, a burst of transmissions is possible. Other than event-triggered approaches, the proposed methods allow to specify the network traffic beforehand by means of the token bucket. Lastly, we validate the proposed approaches in a numerical example.

==> figure/tikz2/tikzbeta_periodic_c8_g3_N3_v2.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.844in,
height=1.55in,
at={(0.813in,0.378in)},
scale only axis,
xmin=0,
xmax=250,
xlabel style={font=\color{white!15!black}},
xlabel={$k$},
ymin=0,
ymax=25,
ylabel style={font=\color{white!15!black}},
ylabel={$\beta(k)$},
axis background/.style={fill=white},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot[const plot, color=mycolor1] table[row sep=crcr] {%
0	22\\
1	22\\
2	17\\
3	12\\
4	12\\
5	7\\
6	2\\
7	2\\
8	5\\
9	0\\
10	0\\
11	3\\
12	6\\
13	6\\
14	9\\
15	12\\
16	12\\
17	15\\
18	18\\
19	18\\
20	21\\
21	22\\
22	22\\
23	22\\
24	22\\
25	22\\
26	22\\
27	22\\
28	22\\
29	22\\
30	22\\
31	22\\
32	22\\
33	22\\
34	22\\
35	22\\
36	22\\
37	22\\
38	22\\
39	22\\
40	22\\
41	22\\
42	22\\
43	22\\
44	22\\
45	22\\
46	22\\
47	22\\
48	22\\
49	22\\
50	22\\
51	22\\
52	22\\
53	22\\
54	22\\
55	22\\
56	22\\
57	22\\
58	22\\
59	22\\
60	22\\
61	22\\
62	22\\
63	22\\
64	22\\
65	22\\
66	22\\
67	22\\
68	22\\
69	22\\
70	22\\
71	22\\
72	22\\
73	22\\
74	22\\
75	22\\
76	22\\
77	22\\
78	22\\
79	22\\
80	22\\
81	22\\
82	22\\
83	22\\
84	22\\
85	22\\
86	22\\
87	22\\
88	22\\
89	22\\
90	22\\
91	22\\
92	22\\
93	22\\
94	22\\
95	22\\
96	22\\
97	22\\
98	22\\
99	22\\
100	22\\
101	22\\
102	22\\
103	22\\
104	22\\
105	22\\
106	22\\
107	22\\
108	22\\
109	22\\
110	22\\
111	22\\
112	22\\
113	22\\
114	22\\
115	22\\
116	22\\
117	22\\
118	22\\
119	22\\
120	22\\
121	22\\
122	22\\
123	22\\
124	22\\
125	22\\
126	22\\
127	22\\
128	22\\
129	22\\
130	22\\
131	22\\
132	22\\
133	22\\
134	22\\
135	22\\
136	22\\
137	22\\
138	22\\
139	22\\
140	22\\
141	22\\
142	22\\
143	22\\
144	22\\
145	22\\
146	22\\
147	22\\
148	22\\
149	22\\
150	22\\
151	22\\
152	22\\
153	22\\
154	22\\
155	22\\
156	22\\
157	22\\
158	22\\
159	22\\
160	22\\
161	22\\
162	22\\
163	22\\
164	22\\
165	22\\
166	22\\
167	22\\
168	22\\
169	22\\
170	22\\
171	22\\
172	22\\
173	22\\
174	22\\
175	22\\
176	22\\
177	22\\
178	22\\
179	22\\
180	22\\
181	22\\
182	22\\
183	22\\
184	22\\
185	22\\
186	22\\
187	22\\
188	22\\
189	22\\
190	22\\
191	22\\
192	22\\
193	22\\
194	22\\
195	22\\
196	22\\
197	22\\
198	22\\
199	22\\
200	22\\
201	22\\
202	22\\
203	22\\
204	22\\
205	22\\
206	22\\
207	22\\
208	22\\
209	22\\
};
\addlegendentry{$\beta(N=3)$}

\end{axis}
\end{tikzpicture}%
